Animatable Implicit Neural Representations for Creating Realistic Avatars from Videos

This paper addresses the challenge of reconstructing an animatable human model from a multi-view video. Some recent works have proposed to decompose a non-rigidly deforming scene into a canonical neural radiance field and a set of deformation fields that map observation-space points to the canonical space, thereby enabling them to learn the dynamic scene from images. However, they represent the deformation field as translational vector field or SE(3) field, which makes the optimization highly under-constrained. Moreover, these representations cannot be explicitly controlled by input motions. Instead, we introduce a pose-driven deformation field based on the linear blend skinning algorithm, which combines the blend weight field and the 3D human skeleton to produce observation-to-canonical correspondences. Since 3D human skeletons are more observable, they can regularize the learning of the deformation field. Moreover, the pose-driven deformation field can be controlled by input skeletal motions to generate new deformation fields to animate the canonical human model. Experiments show that our approach significantly outperforms recent human modeling methods. The code is available at https://zju3dv.github.io/animatable_nerf/.

==> table/01_ablation_studies_pose.tex <==
\begin{table}
\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{100}|x{35}|x{35}}
& PSNR & SSIM \\[.1em]
\shline
Marker-based pose estimation & \textbf{23.72} & \textbf{0.886} \\
Marker-less pose estimation & 22.27 & 0.858 \\
\end{tabular}
\end{center}
\vspace{-1.5em}
\caption{\textbf{Comparison between models trained with human poses} from marker-based and marker-less pose estimation methods on subject ``S9".}
\label{table:human_pose}
\end{table}


==> table/03_supplementary_train_test.tex <==
\begin{table}
\begin{center}
\tablestyle{4pt}{1.05}
\begin{tabular}{x{25}|x{15}|x{15}|x{15}|x{15}|x{15}|x{15}|x{15}}
& S1 & S5 & S6 & S7 & S8 & S9 & S11 \\[.1em]
\shline
training & 150 & 250 & 150 & 300 & 250 & 260 & 200 \\
test & 49 & 127 & 83 & 200 & 87 & 133 & 82 \\
\end{tabular}
\end{center}
\caption{\textbf{Frame numbers for training and test of each subject.}}
\vspace{-0.5em}
\label{table:train_test}
\end{table}


==> teaser.tex <==
%#################################################################################################
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{figure/introduction/teaser}
\end{center} \vspace{-1.5em}
\captionof{figure}{Given a multi-view video of a performer, our method reconstructs an animatable human model, which can be used for novel view synthesis and 3D shape generation under novel human poses.}
\label{fig:teaser}
\end{figure*}
%#################################################################################################

